Extracting Basic Graph Patterns from Triple Pattern Fragment Logs

The Triple Pattern Fragment (TPF) approach is de-facto a new way to publish Linked Data at low cost and with high server availability. However, data providers hosting TPF servers are not able to analyze the SPARQL queries they execute because they only receive and evaluate queries with one triple pattern. In this paper, we propose LIFT: an algorithm to extract Basic Graph Patterns (BGPs) of executed queries from TPF server logs. Experiments show that LIFT extracts BGPs with good precision and good recall generating limited noise.

==> ex1-ctp-extraction.tex <==
\begin{small}
\begin{figure}[t]
  \centering
%%% LOG
\subfloat[Log of $s_1$]{\label{fig:extractlog} 
\begin{tabular}{|l|l|l|} \hline \rowcolor{gray!70}
\multicolumn{3}{|c|}{\textbf{$l_1$: log of $s_1$}} \\ \hline \rowcolor{gray!50}
\textbf{ts} &\textbf{tp} & \textbf{$\mu_o$} \\ \hline
1 & ?s~p1~?o &
\begin{tabular}{l|lll}
?s & s1 & s2 & s3 \\ \hline
?o & o1 & o2 & o3
\end{tabular}
\tikzmark{SQ1} \\ \hline \rowcolor{gray!25}
5 & ?s~p1~o1 &
\begin{tabular}{l|ll}
?s & s1 & s2 \\ 
\end{tabular}
\tikzmark{SQ5}\\ \hline
6 & ?s~p2~?o &
\begin{tabular}{l|ll}
?s & s1 & s2 \\ \hline
?o & o3 & o4 \\
\end{tabular} \tikzmark{SQ6}\\ \hline \rowcolor{gray!25}
7 & ?s~p3~?o &
\begin{tabular}{l|lll}
?s & o1 & o2 & o3 \\ \hline
?o & o4 & o4 & o5 \\
\end{tabular} \tikzmark{SQ7}\\ \hline
8 & s1~p2~?o &
\begin{tabular}{l|l}
?o & o3 \\ 
\end{tabular}
\tikzmark{SQ8}\\ \hline \rowcolor{gray!25}
9 & o3~p3~?o &
\begin{tabular}{l|l}
?o & o5 \\ 
\end{tabular}
\tikzmark{SQ9}\\ \hline
10& s2~p2~?o &
\begin{tabular}{l|l}
?o & o4 \\ 
\end{tabular}
\tikzmark{SQ10} \\ \hline \rowcolor{gray!25}
 11& o4~p3~?o & 
\begin{tabular}{l|l}
?o & $\emptyset$ \\ 
\end{tabular} \tikzmark{SQ11} \\\hline
\end{tabular}}~~~%
%%% CTP NOW
\subfloat[Extracted candidate triple patterns.]{\label{fig:extractctp}
\begin{tabular}{|l|l|l|l|l|} \hline \rowcolor{gray!70}
\multicolumn{5}{|c|}{\textbf{CTP List}} \\ \hline \rowcolor{gray!50}
\textbf{id} & \textbf{ts} &\textbf{tp} & \textbf{$\mu_o$} &\textbf{\begin{tabular}{cc} $\mu_i$ \end{tabular}} \\ \hline
\tikzmark{ctp1} 1 & 1,1 & ?s~p1~?o    
& \begin{tabular}{l|lll}
  ?s & s1 & s2 & s3 \\ \hline
  ?o & o1 & o2 & o3
  \end{tabular} & \\ \hline \rowcolor{gray!25}

\tikzmark{ctp2} 2 & 5,5 &?s~p1~$?o_{in}$    
& \begin{tabular}{l|ll}
  ?s & s1 & s2 \\ 
  \end{tabular}
& \begin{tabular}{l|l}
  $?o_{in}$ & o1 \\ 
  \end{tabular} \\ \hline

\tikzmark{ctp3} 3 & 6,6 & ?s~p2~?o   
& \begin{tabular}{l|ll}
  ?s & s1 & s2 \\ \hline
  ?o & o3 & o4 \\
  \end{tabular}
& \\ \hline \rowcolor{gray!25}

\tikzmark{ctp4} 4 & 7,7 & ?s~p3~?o 
& \begin{tabular}{l|lll}
  ?s & o1 & o2 & o3 \\ \hline
  ?o & o4 & o4 & o5 \\
  \end{tabular}
& \\ \hline

\tikzmark{ctp5} 5 & \cellcolor{red!25}  8,10 & \cellcolor{red!25} $?s_{in}$~p2~?o    
& \begin{tabular}{l|ll}
  ?o & o3 & o4 \\ 
  \end{tabular} 
& \begin{tabular}{l|ll}
  $?s_{in}$ & s1 & s2 \\ 
  \end{tabular} \\ \hline \rowcolor{gray!25}

\tikzmark{ctp6} 6 & \cellcolor{red!25}  9,11 & \cellcolor{red!25} $?s_{in}$~p3~?o    
& \begin{tabular}{l|l}
  ?o & o5  \\ 
  \end{tabular} 
& \begin{tabular}{l|ll}
  $?s_{in}$ & o3 & o4 \\ 
  \end{tabular} \\ \hline
\end{tabular}

\DrawArrow[blue,out=0, in=180]{SQ1}{ctp1}
\DrawArrow[red, out=0, in=180]{SQ5}{ctp2}
\DrawArrow[blue, out=0, in=180]{SQ6}{ctp3}
\DrawArrow[blue, out=0, in=180]{SQ7}{ctp4}
\DrawArrow[blue, out=0, in=180]{SQ8}{ctp5}
\DrawArrow[red, out=0, in=180]{SQ9}{ctp6}
\DrawArrow[blue, out=0, in=180]{SQ10}{ctp5}
\DrawArrow[red, out=0, in=180]{SQ11}{ctp6}}
  \caption{Extraction of candidate triple patterns with gap=3 (the ip column is removed to simplify).}
\label{fig:ctpextraction}
\end{figure}
\end{small}


==> ex2-bgp-extract.tex <==
%NEW algo for nested-loop with split
% \begin{figure}
% \centering
% \begin{tikzpicture}[text centered]
% \matrix(m)[row sep=1.0em,column sep=4em,minimum width=2em] 
% {
%  \node(dtp1){
%  \begin{tabular}{c} 
% $?s~p2~?\omega$ \\
% $dtp[1]$, $\omega=toto$
% \end{tabular}}; & 

% \node(dtp3){
%  \begin{tabular}{c} 
% $?\sigma~p1~?o$ \\
% $dtp[3]$
% \end{tabular}
% }; \\
                                         
% \node(dtp2){
%  \begin{tabular}{c} 
% $?s~p3~?\omega$ \\
% $dtp[2]$, $\omega=titi$
% \end{tabular}};  

% & 
% \node(dtp4){
%  \begin{tabular}{c} 
% $?\sigma~p1~?o$ \\
% $dtp[4]$
% \end{tabular}
% };  \\
%                                        &
%                                        \node(dtp5){
%                                        \begin{tabular}{c} 
%                                          $?\sigma~p4~?\omega$ \\
%                                          $dtp[5], \omega=tata$
%                                        \end{tabular}}; \\
% };
%  \path[*-*]
%    (dtp1) edge node[above]{$?s = ?\sigma$}(dtp3)
%    (dtp2) edge node[above]{$?s = ?\sigma$}(dtp4)
%    (dtp2) edge node[above]{$?s = ?\sigma$}(dtp5)
% ;
% \end{tikzpicture}
% \caption{Connected components of DTPs produced by the execution of the
%   algorithm~\ref{algo:nestedLoopDetection} on the CTPs of
%   figure~\ref{fig:nested-ctp}, for $gap=8$.}
% \label{fig:bgp-extract}
% \end{figure}


\begin{figure}
\centering

\subfloat[\textbf{\{?s1 p2 $toto$ . ?s1 p1 o3\}}]{
\begin{tikzpicture}[ampersand replacement=\&]
\matrix(m)[row sep=1.5em,column sep=4em,minimum width=2em] {
 \node(dtp1){
 \begin{tabular}{c} 
$?s~p2~?\omega$ \\
$dtp[1]$, $\omega=toto$
\end{tabular}};
\& 
 \node(dtp3){
  \begin{tabular}{c} 
 $?\sigma~p1~?o$ \\
 $dtp[3]$
 \end{tabular}
 }; \\ 
};
 \path[-stealth] (dtp1) edge node[above]{$?s = ?\sigma$}(dtp3); 
\end{tikzpicture}
}
%
\subfloat[\textbf{\{?s2 p3 $titi$ . ?s2 p1 ?o4  . ?s2 p4 $tata$\}}]{
\begin{tikzpicture}[ampersand replacement=\&]
\matrix(m)[row sep=0.0em,column sep=4em,minimum width=2em] 
{
\node(dtp2){
 \begin{tabular}{c} 
$?s~p3~?\omega$ \\
$dtp[2]$, $\omega=titi$
\end{tabular}};  
\&  
\node(dtp4){
 \begin{tabular}{c} 
$?\sigma~p1~?o$ \\
$dtp[4]$
\end{tabular}
};  \\

                                      \&
                                       \node(dtp5){
                                       \begin{tabular}{c} \rowcolor{white}
                                         $?\sigma~P3~?\omega$ \\
                                         $dtp[5], \omega=tata$
                                       \end{tabular}}; \\
};
 \path[-stealth]
   (dtp2) edge node[above]{$?s = ?\sigma$}(dtp4)
   (dtp2) edge node[below]{$?s = ?\sigma$}(dtp5)
;

\end{tikzpicture}}
%\caption{Connected components of the DTP graph produced by the execution of 
%  Algorithm~\ref{algo:nestedLoopDetection} on the CTP List of
%  Figure~\ref{fig:nested-ctp}, for $gap=8$.}
\caption{Connected components of the DTP Graph produced by the execution of 
  Algorithm~\ref{algo:nestedLoopDetection} for $gap=8$.}
  
\label{fig:bgp-extract}
\end{figure}


==> pmotiv1.tex <==
%\begin{figure*}[ht!]
%\centering
%\includegraphics[width=50mm,scale=0.5]{
\begin{tikzpicture}
\centering
\tikzstyle{vecArrow} = [thick, decoration={markings,mark=at position
   1 with {\arrow[semithick]{open triangle 60}}},
   double distance=3pt, shorten >= 5.5pt,
   preaction = {decorate},
   postaction = {draw,line width=2pt, white,shorten >= 4.5pt}]

\node(q1)at(-3.5,0)[draw, align=left, rounded corners, text width=8.2cm, %shape=rounded rectangle, minimum width=1.8cm, %drop shadow={opacity=.5,shadow xshift=0pt}
font=\small,label=above:$C_1 (173.28.19.114):$ Query $Q_1$]{
\begin{tabular}{lc}
\textbf{SELECT} ?movie ?title ?name \textbf{WHERE} \{  & \\
?movie ~$dbpedia-owl:starring$ ~?actor  .  & ($tp_1$) \\
?actor ~$rdfs:label$ ~$"Brad~Pitt"@en$ . & ($tp_2$) \\
?movie ~$rdfs:label$ ~?title . &($tp_3$) \\
?movie ~$dbpedia-owl:director$ ~?director . & ($tp_4$) \\
?director ~$rdfs:label$ ~?name   & ($tp_5$) \\

        ~ FILTER LANGMATCHES(LANG(?title), "EN") & \\ 
       ~ FILTER LANGMATCHES(LANG(?name),  "EN") & \}
  \end{tabular}}; 
 
    
    
\node(q2)at(5.5,0)[draw, align=left, rounded corners, text width=8.6cm, %shape=rounded rectangle, minimum width=1.8cm, %drop shadow={opacity=.5,shadow xshift=0pt}
font=\small,label=above:$C_2 (173.28.19.114):$ Query $Q_2$]{
\begin{tabular}{lc}
       \textbf{SELECT} ?titleEng ?title \textbf{WHERE} \{  & \\ 
       ?movie ~$dbpprop:starring$  ~?actor . & ($tp_1$) \\
       ?actor ~$rdfs:label$ ~$"Natalie~Portman"@en$ . & ($tp_2$) \\
       ?movie ~$rdfs:label$ ~?titleEng . & ($tp_3$) \\
       ?movie ~$rdfs:label$ ~?title .  & ($tp_4$) \\ 
        ~ FILTER LANGMATCHES(LANG(?titleEng), "EN") & \\ 
        ~ FILTER (!LANGMATCHES(LANG(?title),  "EN")) & \}
  \end{tabular}};
 

% % % % federation of endpoints

\node (DBPedia) [cylinder,
                cylinder uses custom fill,
                cylinder body fill=blue!20,
                cylinder end fill=blue!20, 
                shape border rotate=90,
                draw,
                 minimum height=0.75cm,
                 minimum width=2.2cm, 
                 label={[align=center]below:DBpedia\\LDF Server}] at (0.5,-2.8) {};



 \path[arrow](q1) edge[red,dashed]  (DBPedia);

 \path[arrow](q2) edge[red,dashed]  (DBPedia);


\end{tikzpicture}
%} 

 %\caption{Query processing and \feta's deduction for CD3, CD4 concurrent execution.}
%	  \label{fig:motivation_example2}
%	\end{figure*}


